Evaluating the False Trust Engendered by LLM Explanations

Large Language Models (LLMs) and Large Reasoning Models (LRMs) are increasingly used for critical tasks, yet they provide no guarantees about the correctness of their solutions. Users must decide whether to trust the model's answer, aided by reasoning traces, their summaries, or post-hoc generated explanations. These reasoning traces, despite evidence that they are neither faithful representations of the model's computations nor necessarily semantically meaningful, are often interpreted as provenance explanations. It is unclear whether explanations or reasoning traces help users identify when the AI is incorrect, or whether they simply persuade users to trust the AI regardless. In this paper, we take a user-centered approach and develop an evaluation protocol to study how different explanation types affect users' ability to judge the correctness of AI-generated answers and engender false trust in the users. We conduct a between-subject user study, simulating a setting where users do not have the means to verify the solution and analyze the false trust engendered by commonly used LLM explanations - reasoning traces, their summaries and post-hoc explanations. We also test a contrastive dual explanation setting where we present arguments for and against the AI's answer. We find that reasoning traces and post-hoc explanations are persuasive but not informative: they increase user acceptance of LLM predictions regardless of their correctness. In contrast, dual explanation is the only condition that genuinely improves users' ability to distinguish correct from incorrect AI outputs.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}
\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We instantiate the evauation protocol in a single domain and test different kinds of explanations, and report our findings,
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have a limitations section in the main text.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We describe the evaluation protocol and study setup in detail, in both appendix and the main text.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Will release later, on acceptance
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or .
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Provided in appendix. We use E⁺/⁻ as the reference condition; results are reported as odds ratios with 95% CIs in Table~\ref{tab:app-glmm}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, we have discussed the positive impact of this evaluation protocol, in measuring false trust engendered in end-users.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, we have cited the papers.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We are not releasing any new assets. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We include all these details in the appendix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerYes{}% Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Study is approved by IRB, and duly declared in the appendix of the paper. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: LLMs are used to generate explanations.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> sections/Conclusion.tex <==
\section{Conclusion}
In this paper, we introduce a novel evaluation protocol to isolate the effects of different explanation conditions on user trust by simulating a setting where users do not have the ability or the means to directly verify the LLM's prediction. We conducted a between-users study where users needed to judge whether a LLM generated answer is correct. We found that reasoning traces, their summaries and post hoc LLM generated answer explanations can hinder the detection of incorrect AI answers and engender false trust in users. In an attempt to mitigate this, we evaluated a post-hoc dual explanation generation paradigm, where users are exposed to both merits and demerits of the LLM's generated answer. We find that the dual explanation condition minimizes false trust while maintaining a high detection accuracy.





==> sections/Introduction.tex <==
%[Start with how traditional AI systems were deep and narrow- had guarentees-thus explanatios nwere need to increase reliance. They did not have a shared vocabulary with humans - outline the problems with xAi pre LLMs]

%There has been a huge shift in the nature of AI systems predominantly available. Traditional AI systems, symbolic or non-symbolic, were deep and narrow systems -- they were experts in one particular task [CITE - Deepblue, AlphaGO?] whereas modern AI systems, particularly generative models, are broad and shallow. Large Language models (LLMs) are the most popular among such systems. LLMs have demonstrated impressive capabilities across a wide array of tasks, from planning and reasoning to instruction following and story writing. However, unlike the traditional systems, they provide no soundness guarantees.

%Narrow systems were good at the task. there could be guarentees. thus various explanations, either symbolic or Space time symbolic tubes were developed so that the human can understand how these systems made decisions
\section{Introduction}
 Traditional AI systems, symbolic or non-symbolic, were deep and narrow systems -- they were experts in one particular task [CITE - Deepblue, AlphaGO?]. The field of Explainable AI (xAI) evolved around these models. Since these models did not share the same internal representations as humans, various explanation techniques were developed to explain the decision making of these systems. The main objective behind the development of these techniques was to faithfully explain the reasoning of the expert system to the user such that the user trust and reliance increases [CITE].



%[Onset of LLMs - Broad and shallow. Share the same representations. Does that means the pre-lLm xai probelms are solved? Identify the new problems that emerge - since there are no guarentees and the system confidently gives answer to everything - how does the user decide when to rely and when not to]

With the advent of Large Language models (LLMs), the field of AI has been revolutionized. LLMs have demonstrated impressive capabilities across a wide array of tasks, from planning and reasoning to instruction following and story writing [CITE]. Unlike traditional AI systems, these generative language models are broad and general purpose models. When prompted with a question, regardless of the problem domain or complexity, LLMs will confidently provide an answer. However these systems come with a caveat, there are no guarantees that the generated answer will be correct. With their growing use, users are increasingly prompting these models with critical questions regarding healthcare, education, legal, etc and the onus is on the prompter whether to trust the system or not.

%Since there are no correctness guarantees, there is a paramount need for developing explanation generation paradigms that will help the users in identifying when the LLM is incorrect.

%[Types of explanations - Reasoning models - reasoning trace. currently we dont know how the tokens displayed to the users are generated - post hoc or summary? how this the popular mode. post-hoc explanations why it might be correct. Cite works which say how the reasoning traces are not faithfull representations of models computations. Thus trace and summary cannot be faithfull explanations of how the model came to its predicted answer. Post hoc does not even have the reasoning so no reason to expect that it will be faithful]

Recently, a new crop of language models called Large Reasoning Models (LRMs) have emerged. These reasoning models, when presented with a question, generate a sequence of intermediate tokens (colloquially or perhaps fancifully called a “Chain of Thought” or “reasoning trace”) before producing an answer sequence [CITE]. These reasoning traces have often been interpreted as the intermediate steps which the model took to arrive at the final answer. This has led the community to believe that these reasoning traces can be treated as \textbf{provenance explanations} [CITE]. However, none of the major frontier model makers–OpenAI, Google, Anthropic [CITE]- show the actual reasoning traces which the models produced. They only show  what seems like a summarized version of the actual intermediate tokens. GPT-OSS models [CITE] have a high level commentary tokens which are interpretable for the end user, and is admittedly distinct from the analysis part that corresponds to intermediate tokens. These commentary tokens might very well have been generated post-hoc to explain the LLM's predicted answer.
%It is not clear how these sumarries and and commentary parts are generated. 
Some researchers have cautioned against interpreting these reasoning traces as faithful representations of the model's internal computations [CITE]. Researchers have also demonstrated how these reasoning traces do not need to have any semantics or any end-user interpretability [CITE]. 


%[Motivated by the above - we want to see what are the effects of the exposing these kinds of explanations to users in a setting where the system accuracy is not near perfect and the user does not have the ability to verify the solution. Specifically, we want to check whether users are able to able to distinguish between correct and incorrect AI predictions given these different explanation conditions. we emphasize on measuring the false trust - the number of times users end up trusting an incorrect AI prediction as correct. -- Motivate how this might be the most dangerous - AI systems exploiting our cognitive beliefs [might also add the sycophantic work]. Motivate the e\_dual condition - as showing pros and cons to the user].

%[study design] 

In light of these recent findings, our study is aimed at understanding the effects of exposing the various kinds of explanations of LLM generated answers to users in a setting where the model's accuracy is not near perfect and the user does not have the ability to verify the solution. Concretely, we conduct a between-subjects user study where participants are shown questions, their LLM generated answers, and vary the type of explanation which the users are exposed to. The goal of the participants is to distinguish between a correct and an incorrect LLM generated answer. We conduct our study on challenging math, physics and chemistry problems from the JEE-Bench dataset [CITE]. We want to examine whether the different explanation paradigms are potentially exploiting the cognitive flaws of lay users, convincing them of the validity of incorrect answers. Thus, we focus on measuring the false trust engendered in users - the number of times users trust an incorrect AI prediction as correct. The results of our pilot study demonstrated that the rate of false trust engendered in participants was significantly higher compared to our baseline where no explanation was provided. As a \textit{first attempt} to mitigate this critical issue, we propose a new post hoc explanation generation paradigm - \textit{e\_dual}, where the user is exposed to the merits and demerits of the LLM generated answer.




[Results para - motivate the appropriate trust measure. Our results show that showing the reasoning trace summary and e\_plus is the induce most false trust. Next we check the appropriate trust and find that e\_dual and reasoning trace have the highest accuracy.  We further study how the users which have some domain knowledge but not enough to solve the question benefit the most with e\_dual. Additionally we show how not all explanations are equally helpful to the users; point out how reasoning traces have the highest cognitive load [cite -traceinterp]] and how their utility arises from being exceptionally bad for incorrect answers. In the end point out how e\_dual mech is a good possible alternative - we find that e\_dual conditions provides higherst approipriate trust, users find it helpful, most beneficial when users have partial knowledge]

[Ending - caution against interpreting reasoning trace and their summary as provenance explanations since they are not faithful representations. post-hoc explanations need to be balanced and not designed to gaslight users. E\_dual is one possible mech - there can be better ones.]

==> sections/Methodology.tex <==
\section{Methodology}
\textbf{Dataset: }We conduct evaluation on the JEE-Bench dataset [CITE]. JEE-Bench is a challenging dataset consisting of 515 preengineering mathematics, physics, and chemistry curated problems from the highly competitive IIT JEE-Advanced exam. We chose a challenging dataset because we wanted non-trivial problems where users could not simply verify the correctness of an LLM-generated answer by solving the problems themselves and ignoring the explanations or reasoning provided with the LLM-generated answers [CITE].

\textbf{Models: }We used Deepseek R1[CITE] to generate responses on JEE-Bench problems since Deepseek R1 provides access to the model's intermediate tokens unlike other closed source reasoning models. Thus, R1 generated responses contain reasoning traces and the final answer. We use Gpt 4o-mini [CITE] to generate the summaries of the reasoning traces produced by R1. We use Deepseek V3 [Cite] for generating the explanations on R1 generated answers. We provide the prompt templates used in each condition in the Appendix [to-do].

\subsection{User-study}
We conducted user-studies across 5 different conditions to evaluate the engendered user-trust across various paradigms.
Participants were recruited via Prolific and the study was reviewed and approved by the Institutional Review Board (IRB). [WRITE ABOUT PARTICIPANT QUALIFICATIONS.]
In each condition, participants were shown 8 problems drawn from physics, chemistry, and mathematics. The AI system's accuracy on the selected items was 50\% (4 correct and 4 incorrect answers per participant). Of the 8 items, 4 were \emph{fixed} questions that were kept constant across all participants and conditions. The remaining 4 were \emph{sampled} questions, randomly drawn from the full dataset of correctly and incorrectly answered questions, with 2 correct and 2 incorrect answers per participant. 


Participants received a base pay of \$3.00 and could earn a performance bonus of up to \$2.00 based on the accuracy of their judgments of the AI's answers (\$0.25 per correct judgment across 8 items), for a maximum total of \$5.00. This incentive structure was designed to encourage careful evaluation of the AI's outputs. The expected study duration was approximately 20 minutes.
 

==> sections/ack.tex <==
\section*{Acknowledgments}
This research is supported in part by grants from ONR (N00014-25-1-2301 and N00014-23-1-2409), DARPA (HR00112520016), DoD RAI (via CMU subcontract 25-00306-SUB-000), and a generous gift from Qualcomm.

==> sections/discussion.tex <==
\section{Discussion}
%[Emphasize how this is a necessary evaluation protocol and how it is setup and it is the first human-centred study.]
\subsection{Necessity of the evaluation protocol}
In this paper, we introduce a novel evaluation protocol to evaluate LLM-generated explanations. 
%the following can be shortened
Since LLM generated answers never have any guarantees, the burden of verification of correctness is on the user. 
%Currently one of the predominant paradigms, with the onset of Chain of thought prompting or Reasoning models, LLMs have started generating reasoning traces which supposedly reflect the intermediate computations the model did to generate the solution. 
Most frontier models [CITE] generate either reasoning traces or commentary tokens which can be summaries of reasoning traces or post-hoc explanations of the LLM generated answers. The reasoning traces, their summaries or LLM generated answer's post-hoc explanations are exposed to the user. It is established that reasoning traces help the LLM perform better, but it is not studied what effect these traces have on the end-user. Thus we believe that it is crucial to study the effects of exposing these traces to the end-user. Moreover, it is necessary to evaluate whether any of these explanation conditions engenders false trust in users and persuades them to trust incorrect LLM-generated answers.
%Given the recent evidence, we wanted to evaluate what effect d. We believe that

%In our study, users need to judge whether a LLM generated answer is correct. We carefully simulate a setting where users do not have the means to directly verify the solution and must engage with the provided explanation. This enabled us to isolate the causal impact of the provided explanations on user persuasion. 
 

%Our study simulates a setting where the User does not have the means to verify the solution and is aided

\subsection{Reasoning traces and their summaries can hinder the detection of incorrect AI answers}
As observed in Sections 4.1 and 4.2, Reasoning traces and their summaries have high false trust and misjudgement rates. This means that a user, when exposed to a reasoning trace or its summary leading to an incorrect prediction, it is more likely to believe that the answer is correct. Our speculation is that this is happening because users are likely to see familiar phrases in reasoning traces, reminiscent of what a human solving such a problem might utter, and assume that the reasoning trace sounds plausible and thus the generated answer must be correct. 
This tendency is so irresistible that even researchers, based on qualitative analyses of the trace contents, have hypothesized that reasoning traces improve LLMs performance by instilling cognitive behaviors [CITE].
However, recent work [CITE] that there is only a loose correlation between the correctness of the trace and the answer correctness. In [CITE FAIThfullness works], researcher have also shown that the Language models are not always faithfull to their reasoning traces. Thus, this disconnect between the seemingly plausible reasoning trace and the final solution correctness increases the false trust and misjudgement rates in users.


% RLHF to be persuasive \\

\subsection{Explanations should reflect the model's uncertainty}
%Ideally, we want explanations that are faithful to the model's reasoning and reflect the model's uncertainty in the generated answer. [CITE?]
%This enables users to distrust the model's answer when a confidently predicted answer is achieved through incorrect reasoning or the model itself is unsure of the predicted answer. 
%It is unclear how to get explanations that are faithful to the model's reasoning [CITE]. 
It is established that displaying the uncertainty in AI's predictions can help users to distinguish between correct and incorrect answers [CITE]. However, it is not established how to quantify an LLM's uncertainty, with different researchers proposing various metrics [CITE]. We posit that LLM generated explanations should reflect model's uncertainty to the user
As a \textit{first attempt} to , we propose a new post hoc explanation generation paradigm - \textit{e\_dual}, where the user is exposed to the merits and demerits of the LLM generated answer.
%the explanation generation paradigms with LLMs, either reasoning trace or their summaries or the post-hoc explanation generation do not faithfully reflect the internal computations of the model [CITE- faithfullness works]

[Appropriate trust findings - say e\_dual is a first attempt to solve the problem of the appropriate trust. since anyway reasoning trace and post\_hoc explanations are not faithfull explanations of models answer, we can have different explanation generation methods - e\_dual being one of them. Most helpful when the user is somewhat familiar with the problem - then e\_dual helps the most. this is the exact case where users can engage with the explanations and make an informed choice when presented with pros and cons]

\textcolor{red}{Do we need to add a Limitations section?}



==> sections/intro_v2.tex <==
\section{Introduction}
With the advent of Large Language models (LLMs), the field of AI has been revolutionized. LLMs have demonstrated impressive capabilities across a wide array of tasks, from planning and reasoning to instruction following and story writing [CITE]. Unlike traditional AI systems, these generative language models are broad and general purpose models, leading to their rapid adoption by lay users. 
However, this adoption comes with a caveat.
Large Language Models confidently answer any question put to them, regardless of whether the answer is correct. As these systems are increasingly used for critical decisions in healthcare, education, and legal domains, a fundamental question emerges: how does the user decide when to trust the system and when not to?

Traditional Explainable AI (xAI) technique were designed for deep and narrow, task-specific AI systems that were experts in one domain [CITE — DeepBlue, AlphaGo]. Since they did not share the same internal representations as humans, these systems were reliable but opaque. The goal of showing explanations to users was therefore to increase user trust by faithfully explaining the system's decision-making process [CITE]. LLMs invert this problem. These systems are not opaque but unreliable. They communicate in natural language and readily provide an explanation of their decision making, while not providing any guarantees of correctness. The xAI challenge is no longer ``how do we get users to trust an opaque system?'' It is ``how do we help users calibrate their trust in an unreliable system?''


Recently, a new crop of language models called Large Reasoning Models (LRMs) have emerged. These reasoning models, when presented with a question, generate a sequence of intermediate tokens (colloquially or perhaps fancifully called a “Chain of Thought” or “reasoning trace”) before producing an answer sequence [CITE]. These reasoning traces have often been interpreted as the intermediate steps which the model took to arrive at the final answer, leading the community to treat them as \textbf{provenance explanations} [CITE]. Ironically, none of the major frontier model makers–OpenAI, Google, Anthropic [CITE]- show the actual reasoning traces which the models produced. They only show  what seems like a summarized version of the actual intermediate tokens. GPT-OSS models [CITE] have a high level commentary tokens which are interpretable for the end user, and is admittedly distinct from the analysis part that corresponds to intermediate tokens. These commentary tokens might very well have been generated post-hoc to explain the LLM's predicted answer. Furthermore, researchers have cautioned against interpreting reasoning traces as faithful representations of the model's internal computations [CITE], and have demonstrated that these traces do not need to have any semantic meaning or end-user interpretability to produce correct answers [CITE]. 

In light of these recent findings, we want to study the effects of exposing different kinds of LLM explanations along with their predicted answers in a setting where the model's accuracy is far from perfect and users lack the domain expertise to independently verify the answers predicted by LLM. 
We conduct a between-subjects user study where participants are shown challenging math, physics, and chemistry problems from the JEE-Bench dataset [CITE] alongside LLM-generated answers. We expose users to different types of explanations alongside AI-generated answers: reasoning traces, their summaries, and post-hoc explanations arguing for the answer's correctness. For each question, participants judge whether the AI's predicted answer is correct or incorrect. We focus on measuring false trust engendered in the users i.e. when users trust the AI's answer, how often are they trusting an incorrect answer?

Our pilot study revealed that reasoning traces and post-hoc explanations significantly increased false trust engendered in users, as compared to our baseline where no explanation was provideded. Motivated by this finding, we propose \texttt{e\_dual} — a post-hoc explanation paradigm that presents both the merits and demerits of the AI-generated answer.


[Results para - motivate the appropriate trust measure. Our results show that showing the reasoning trace summary and e\_plus is the induce most false trust. Next we check the appropriate trust and find that e\_dual and reasoning trace have the highest accuracy.  We further study how the users which have some domain knowledge but not enough to solve the question benefit the most with e\_dual. Additionally we show how not all explanations are equally helpful to the users; point out how reasoning traces have the highest cognitive load [cite -traceinterp]] and how their utility arises from being exceptionally bad for incorrect answers. In the end point out how e\_dual mech is a good possible alternative - we find that e\_dual conditions provides higherst approipriate trust, users find it helpful, most beneficial when users have partial knowledge]

[Ending - caution against interpreting reasoning trace and their summary as provenance explanations since they are not faithful representations. post-hoc explanations need to be balanced and not designed to gaslight users. E\_dual is one possible mech - there can be better ones.]

==> sections/results.tex <==
\section{Results}

\subsection{False vs Earned Trust}
For each participant we count how often they said the AI was correct, separately on the items where the AI was actually right and on the items where it was wrong. Earned trust is the fraction correct on the AI-right items i.e. how often the participant accepts a correct answer. False trust is the fraction "correct" on the AI-wrong items i.e. how often the participant accepts an incorrect answer. 
Let participant $i$ judge items $\mathcal{I}_i$ with ground truth
$a_{ij}\in\{1,0\}$ and judgment $\hat y_{ij}\in\{1,0\}$. Let
$\mathcal{I}_i^{+}=\{j:a_{ij}=1\}$ be the AI-correct items shown to $i$ and
$\mathcal{I}_i^{-}$ the AI-incorrect items. Per-participant
\emph{earned trust} ($\mathrm{ET}_i$) and \emph{false trust}
($\mathrm{FT}_i$) are
\begin{equation}
\underbrace{\mathrm{ET}_i = \frac{1}{|\mathcal{I}_i^{+}|}
   \sum_{j\in\mathcal{I}_i^{+}}\hat y_{ij}}_{\text{earned trust}}
\qquad
\underbrace{\mathrm{FT}_i = \frac{1}{|\mathcal{I}_i^{-}|}
   \sum_{j\in\mathcal{I}_i^{-}}\hat y_{ij}}_{\text{false trust}}
\label{eq:trust-defs}
\end{equation}
\begin{table}[t]
\centering
\caption{Earned and false trust rates per explanation condition, split by item
subset (fixed items shown to every participant; randomly sampled items drawn
per participant; pooled = all 8 items). Cells are participant-mean rates in
percent. \textbf{Bold} marks the best cell in each column (highest earned
trust, lowest false trust). $N_{\text{participants}}=24$--$25$ per condition.}
\label{tab:headline}
\small
\begin{tabular}{l rrr rrr}
\toprule
& \multicolumn{3}{c}{\textbf{Earned trust} ($\uparrow$)} & \multicolumn{3}{c}{\textbf{False trust} ($\downarrow$)} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
Condition & Fixed & Sampled & Pooled & Fixed & Sampled & Pooled \\
\midrule
\texttt{solution\_only}     & 56.2 & 64.6 & 60.4 & 60.4 & \textbf{47.9} & 54.2 \\
\texttt{e\_plus}            & 70.0 & \textbf{78.0} & 74.0 & 58.0 & 58.0 & 58.0 \\
\texttt{e\_dual}            & 66.7 & 68.8 & 67.7 & \textbf{45.8} & \textbf{47.9} & \textbf{46.9} \\
\texttt{reasoning\_summary} & 60.0 & 72.0 & 66.0 & 52.0 & 50.0 & 51.0 \\
\texttt{reasoning\_trace}   & \textbf{76.0} & 74.0 & \textbf{75.0} & 56.0 & 52.0 & 54.0 \\
\bottomrule
\end{tabular}
\end{table}


\subsection{Appropriate Trust}
The previous section talked about earned and false trust rates, which gives us independent insights on how users behave on correctly and incorrectly answered questions. However, these rates alone do not tell us whether
users can actually distinguish between the two. A user who simply judged every answer to be correct achieves highest earned trust and highest false trust, while a user who simply judged every answer to be wrong achieves lowest false trust and lowest earned trust. Neither is desirable as we want the explanations to help users accept correct answers \textit{and} reject incorrect answers. To assess which condition helped users actually \emph{distinguish} correct from incorrect AI answers, we frame each participant's judgment as a binary classification problem and report standard confusion matrix metrics (Table ~\ref{tab:h2-confusion}). 
\begin{itemize}
    \item \textbf{Accuracy} $= \frac{TP + TN}{TP + TN + FP + FN}$.
    Fraction of judgments where the user correctly identified whether the AI was right or wrong.

    \item \textbf{Precision} $= \frac{TP}{TP + FP}$.
    When a user judges the AI's answer to be correct, how often is the AI actually correct? Low precision means the user's endorsement is unreliable.

    \item \textbf{Recall} $= \frac{TP}{TP + FN}$.
    How many correct AI answers did the user successfully judge to be correct? Identical to earned trust (Eq.~\ref{eq:trust-defs}).

    \item \textbf{F1} $= \frac{2 \cdot \text{Precision} \cdot
    \text{Recall}}{\text{Precision} + \text{Recall}}$. Balances precision and recall, but does not penalize false trust directly.

    \item $\mathbf{F_{\beta}}$ $= (1+\beta^{2})\cdot \frac{\text{Precision} \cdot \text{Recall}}{\beta^{2}\cdot\text{Precision} + \text{Recall}}$.We report $F_{0.5}$ as being relevant to settings where a user judging an incorrect AI answer as correct is costlier than judging a correct AI answer as incorrect.
\end{itemize}
\begin{table}[t]
\centering
\caption{Confusion-matrix metrics per condition (pooled items).
Precision, recall, and accuracy are in percent; F1 and
F$_{0.5}$ are unitless. F$_{0.5}$ weights precision over recall
($\beta{=}0.5$). \textbf{Bold} = best in column.}
\label{tab:h2-confusion}
\small
\begin{tabular}{l rrrrr}
\toprule
Condition & Precision & Recall & F1 & F$_{0.5}$ & Accuracy \\
\midrule
\texttt{solution\_only}     & 53.3 & 60.9 & .569 & .547 & 53.8 \\
\texttt{e\_plus}            & 56.2 & 75.0 & .643 & .592 & 58.3 \\
\texttt{e\_dual}            & \textbf{59.1} & 67.7 & .631 & \textbf{.606} & \textbf{60.4} \\
\texttt{reasoning\_summary} & 55.4 & 64.6 & .596 & .570 & 56.2 \\
\texttt{reasoning\_trace}   & 57.9 & \textbf{76.0} & \textbf{.658} & .589 & \textbf{60.4} \\
\bottomrule
\end{tabular}
\end{table}
At first glance, \texttt{reasoning\_trace} appears to be the strongest condition: it achieves the highest F1 (.658) and MCC
($+.219$). However, \texttt{reasoning\_trace} and \texttt{e\_plus} both achieve high recall by shifting users toward saying 
``correct'' more frequently, on both correct \emph{and} incorrect items. In contrast, \texttt{e\_dual} is the only condition that reduces false trust below the \texttt{solution\_only} baseline while raising earned trust above it, achieving the highest precision (59.1\%) and tying for the highest accuracy (60.4\%). The MCC gap between \texttt{reasoning\_trace} ($+.219$) and \texttt{e\_dual} ($+.211$)
 is negligible ($\Delta = .008$).
\textcolor{red}{Why do reasoning traces do better?}
Cite beyond semantics and coginterp work. We have evidence that reasoning traces do not need to have any semantic meaning and are also less interpretable. 
\subsection{Perceived Helpfulness}
After each item, participants rated whether the explanation helped them understand how the AI reached its answer. \texttt{solution\_only} provided no explanation and is omitted from this analysis.
Firstly, we find that only 56.8\% of \texttt{reasoning\_trace} responses were rated helpful, compared to 62.5\% for \texttt{reasoning\_summary}, 72.4\% for \texttt{e\_dual} and 82.3\% for \texttt{e\_plus}. Secondly, we split each condition by this rating and compute earned trust, false trust, and accuracy for each group
(Table~\ref{tab:helpfulness}). We discuss the two important findings from our analysis.  

For \texttt{reasoning\_trace} and \texttt{reasoning\_summary}, perceived helpfulness is associated with users accepting the AI's answer indiscriminately. Users who rated the reasoning trace as helpful show 90.0\% earned trust but 85.7\% false trust. The reasoning summary shows the same pattern where the ``helpful'' group
has 82.3\% earned trust alongside 74.1\% false trust. Users accepted nearly every AI answer regardless of whether it was correct. Their accuracy is lower than the ``not helpful'' group  in both cases. Users who reported that reasoning traces and summaries helped them were, in fact, the least accurate. The \texttt{e\_dual} condition is the only case where this relationship is reversed. Users who found the dual explanation helpful achieve 72.6\% earned trust while maintaining 45.5\% false trust. This is desirable as earned trust rises while false trust does not, as compared to users who reported not being helped. Users who reported being helped also had higher accuracy than users who reported they weren't helped. Therefore, in this case, perceived helpfulness corresponds to improved judgment of user.
\begin{table}[t]
\centering
\caption{Earned trust, false trust, and accuracy for each condition compared by
perceived helpfulness. $N$ = item responses per subgroup.
\texttt{solution\_only} omitted (no explanation).}
\label{tab:helpfulness}
\small
\begin{tabular}{l l r rrr}
\toprule
Condition & Perceived helpfulness & $N$ & Earned trust & False trust & Accuracy \\
\midrule
\multirow{2}{*}{\texttt{e\_plus}}
  & Helpful     & 158 & 80.0 & 60.3 & 60.1 \\
  & Not helpful &  34 & 50.0 & 50.0 & 50.0 \\
\midrule
\multirow{2}{*}{\texttt{e\_dual}}
  & Helpful     & 139 & 72.6 & 45.5 & \textbf{64.0} \\
  & Not helpful &  53 & 52.2 & 50.0 & 50.9 \\
\midrule
\multirow{2}{*}{\texttt{reasoning\_summary}}
  & Helpful     & 120 & 82.3 & 74.1 & 55.0 \\
  & Not helpful &  72 & 32.4 & 18.4 & 58.3 \\
\midrule
\multirow{2}{*}{\texttt{reasoning\_trace}}
  & Helpful     & 109 & 90.0 & 85.7 & 56.0 \\
  & Not helpful &  83 & 52.8 & 23.4 & 66.3 \\
\bottomrule
\end{tabular}
\end{table}

\subsection{User Knowledge}
Before seeing the AI's answer, participants rated their familiarity with each problem (``I know the answer immediately,'' ``I might be
able to solve it given more time,'' or ``I cannot solve this''). Table~\ref{tab:knowledge} shows earned trust, false trust, and accuracy for each condition split by this self-reported knowledge level.
Of the responses where users claimed to know the answer immediately, only 37\% were actually correct (33 of 90). We verified this by comparing users' own answers against the answer key. These actually knowledgeable users who answered it correctly achieved just 26.3\% false trust and 84.8\% accuracy. Users who claimed knowledge but answered incorrectly showed 52.0\% false trust, no better than users who reported being unable to solve the problem at all (56.9\%). Across most conditions, higher knowledge is associated with lower false trust and we observe that users who recognize the problem are better at catching incorrect AI answers. 
\begin{table}[t]
\centering
\caption{Earned trust, false trust, and accuracy by knowledge
subgroup (pooled across conditions). ``Actually correct'' and
``actually wrong'' are subgroups of users who claimed to know
the answer immediately (knowledge level 1), split by whether
their own answer matched the answer key.}
\label{tab:knowledge-verified}
\small
\begin{tabular}{l r rrr}
\toprule
Knowledge subgroup & $N$ & Earned trust & False trust & Accuracy \\
\midrule
Claimed knowledge, actually correct & 33 & \textbf{100.0} & \textbf{26.3} & \textbf{84.8} \\
Claimed knowledge, actually wrong   & 57 & 81.2 & 52.0 & 66.7 \\
Might be able to solve it           & 449 & 65.5 & 51.9 & 57.2 \\
Cannot solve this                   & 413 & 68.7 & 56.9 & 55.2 \\
\bottomrule
\end{tabular}
\end{table}

However, \texttt{reasoning\_trace} is the only condition where this pattern reverses. Among users who reported knowing the answer immediately, false trust is 75.0\%, which is higher than any other condition at any knowledge level. For comparison, \texttt{solution\_only} users with the same knowledge level show just 38.9\% false trust. More knowledgeable users appear to follow the chain-of-thought more fluently, which makes it more convincing even when it leads to a wrong answer. Among users who reported partial knowledge (``might be able to solve it''), which is the largest subgroup in our data, \texttt{e\_dual}
achieves 33.3\% false trust and the highest accuracy (64.0\%). This suggests that these kind of explanations are most effective when users have
enough domain knowledge to evaluate the competing arguments. 
\begin{table}[t]
\centering
\caption{Earned trust, false trust, and accuracy for each condition
compared by self-reported knowledge level. $N$ = item responses per
subgroup. Before seeing the AI's answer, participants were asked:
``Do you know how to solve this question?''
(1 = ``I know the answer immediately,''
2 = ``I might be able to solve it given more time,''
3 = ``I cannot solve this'').}
\label{tab:knowledge}
\small
\begin{tabular}{l l r rrr}
\toprule
Condition & Knowledge level & $N$ & Earned trust & False trust & Accuracy \\
\midrule
\multirow{3}{*}{\texttt{solution\_only}}
  & I know it       &  33 & 100.0 & 38.9 & 78.8 \\
  & Might solve it  &  94 &  52.1 & 56.5 & 47.9 \\
  & Cannot solve    &  57 &  55.2 & 57.1 & 49.1 \\
\midrule
\multirow{3}{*}{\texttt{e\_plus}}
  & I know it       &  13 & 100.0 & 42.9 & 76.9 \\
  & Might solve it  &  99 &  72.7 & 54.5 & 60.6 \\
  & Cannot solve    &  80 &  74.3 & 64.4 & 52.5 \\
\midrule
\multirow{3}{*}{\texttt{e\_dual}}
  & I know it       &  13 &  62.5 & 40.0 & 61.5 \\
  & Might solve it  &  89 &  61.4 & \textbf{33.3} & \textbf{64.0} \\
  & Cannot solve    &  90 &  75.0 & 60.9 & 56.7 \\
\midrule
\multirow{3}{*}{\texttt{reasoning\_summary}}
  & I know it       &  20 &  80.0 & 30.0 & 75.0 \\
  & Might solve it  &  80 &  60.0 & 60.0 & 51.2 \\
  & Cannot solve    &  92 &  65.9 & 51.0 & 56.5 \\
\midrule
\multirow{3}{*}{\texttt{reasoning\_trace}}
  & I know it       &  11 &  85.7 & 75.0 & 63.6 \\
  & Might solve it  &  87 &  81.4 & 56.8 & 62.1 \\
  & Cannot solve    &  94 &  69.6 & 52.1 & 58.5 \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Self-reported Trust vs Appropriate Trust}

After completing all items, participants rated their overall trust in the AI on a 7-point scale. We examine whether this self-reported trust measure tracks how well-calibrated the user's judgment is.
Table~\ref{tab:trust-vs-calibration} splits participants by their self-reported trust level. Users who report higher trust show higher earned trust (55.5\% to 89.6\%) and higher false trust (39.0\% to 71.9\%) but their accuracy is unchanged (58.2\%, 57.2\%, 58.9\%). Self-reported trust predicts how often users say ``correct,'' not
how often they are right. Formally, self-reported trust has no correlation with accuracy (Pearson $r = 0.037$, $p = .686$) but is strongly correlated with false trust ($r = 0.409$, $p < .001$).
  
We find that \texttt{reasoning\_trace} elicits the highest self-reported trust (4.44/7) but has higher false trust (54.0\%). 
\texttt{e\_plus} follows the same pattern: second-highest self-reported trust (4.19/7) and the highest false trust of any condition (58.0\%). Both formats provide one-sided reasoning and users respond by reporting high trust but accept incorrect answers.
\texttt{e\_dual} elicits below-average
self-reported trust (3.74/7) but achieves the lowest false trust of any condition (46.9\%). If explanations were evaluated by user satisfaction alone, the format that best calibrates trust would rank near the bottom. Self-reported trust measures how persuasive users found the explanation, not how well it actually helped them judge the AI's answers.

(Table~\ref{tab:trust-mismatch}).
\begin{table}[t]
\centering
\caption{Earned trust, false trust, and accuracy split by
self-reported trust level (post-study, 7-point scale, binned).
Higher self-reported trust is associated with higher earned
trust \emph{and} higher false trust, while accuracy remains
flat. $N$ = number of participants.}
\label{tab:trust-vs-calibration}
\small
\begin{tabular}{l r rrr}
\toprule
Self-reported trust & $N$ & Earned trust & False trust & Accuracy \\
\midrule
Low (1--3)     & 43 & 55.5 & \textbf{39.0} & 58.2 \\
Medium (3.5--5) & 55 & 69.9 & 55.6 & 57.2 \\
High (5.5--7)  & 25 & \textbf{89.6} & 71.9 & \textbf{58.9} \\
\bottomrule
\end{tabular}
\end{table}
\begin{table}[t]
\centering
\caption{Conditions ranked by self-reported trust (post-study,
7-point scale) vs.\ actual false trust and accuracy. Self-reported
trust ranks explanation formats by persuasiveness, not by
calibration quality.}
\label{tab:trust-rankings}
\small
\begin{tabular}{l rrr}
\toprule
Condition & Self-reported trust & False trust ($\downarrow$) & Accuracy ($\uparrow$) \\
\midrule
\texttt{reasoning\_trace}   & \textbf{4.44} & 54.0 & \textbf{60.5} \\
\texttt{e\_plus}            & 4.19 & 58.0 & 58.0 \\
\texttt{e\_dual}            & 3.74 & \textbf{46.9} & 60.4 \\
\texttt{reasoning\_summary} & 3.68 & 51.0 & 57.5 \\
\texttt{solution\_only}     & 3.67 & 54.2 & 53.1 \\
\bottomrule
\end{tabular}
\end{table}

==> sections/results_v3.tex <==
\section{Results}
\subsection{Evaluation Framework}

For each question across every condition, we asked the participant whether they thought the AI's predicted answer was correct. We can compare the user's perceived correctness of the AI's answer with the ground truth. For each participant, we count how often they said the AI was correct, separately on the items where the AI was actually right and on the items where it was wrong. We organize these possible outcomes into a confusion matrix (Fig.~\ref{fig:confusion-pooled}. We derive two complementary sets of metrics as described below.
\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{sections/figs/confusion_pooled.png}
\caption{Pooled confusion matrices per explanation condition.}
\label{fig:confusion-pooled}
\end{figure}
\subsubsection{Trust and Mistrust}
We condition on the user's trust in the system. For every instance where the user chose to trust the AI i.e. judged the AI's answer as correct, we check whether the AI was actually correct or not. Similarly, for every instance where the user chose to mistrust the AI i.e., judged the AI's answer as incorrect, we check whether the AI was actually incorrect or not. This gives us the following metrics: 
% We note that these correspond to what ~\citet{hoffman2023measures} and~\cite{jacovi2021formalizing} call warranted and unwarranted trust respectively.
 
\begin{table}[h]
\centering
\small
\begin{tabular}{lcc}
\toprule
 & \textbf{AI actually correct} & \textbf{AI actually incorrect} \\
\midrule
\textbf{User judged correct}   & True Trust  & False Trust \\
\textbf{User judged incorrect} & False Mistrust & True Mistrust \\
\bottomrule
\end{tabular}
\caption{Trust and mistrust outcomes. Each row conditions on the user's judgment: the trust row (user judged correct) sums across AI-correct and AI-incorrect cases to give the total number of times the user trusted the AI; the mistrust row does the same for distrust.}
\label{tab:trust-matrix}
\end{table}
 
\begin{itemize}
    \item \textbf{True Trust} $= \frac{|\{\text{user judged as correct} \cap \text{AI actually correct}\}|}{|\{\text{user judged as correct}\}|}$.
    Of all the instances where the user trusted the AI, the fraction where the AI was actually correct. A high true trust rate means that when the user decides to trust, that trust is usually well-placed.
 
    \item \textbf{False Trust} $= \frac{|\{\text{user judged as correct} \cap \text{AI actually incorrect}\}|}{|\{\text{user judged as correct}\}|}$.
    Of all the instances where the user trusted the AI, the fraction where the AI was actually incorrect. A high false trust rate means the user is frequently placing trust in wrong answers. True trust and false trust are complements and sum to one.
 
    \item \textbf{False Mistrust} $= \frac{|\{\text{user judged as incorrect} \cap \text{AI actually correct}\}|}{|\{\text{user judged as incorrect}\}|}$.
    Of all the instances where the user mistrusted the AI, the fraction where the AI was actually correct. A high false mistrust rate means the user is rejecting good answers.
 
    \item \textbf{True Mistrust} $= \frac{|\{\text{user judged as incorrect} \cap \text{AI actually incorrect}\}|}{|\{\text{user judged as incorrect}\}|}$.
    Of all the instances where the user mistrusted the AI, the fraction where the AI was actually incorrect. A high true mistrust rate means that when the user decides to reject the AI's answer, that rejection is usually justified. True mistrust and false mistrust are complements and sum to one.
\end{itemize}
 
These metrics tell us whether, when the user chose to trust or mistrust an AI answer based on the explanation shown, that trust was warranted. An explanation that makes users trust more will lower false trust and raise true trust, even if the user is no better at detecting incorrect answers. An explanation that better calibrates the trust of the user will lower false trust while also raising true mistrust.
\label{sec:eval-framework:trust}

\subsubsection{Correct-judgement and Mis-judgement}
We condition on AI correctness to understand how well users can \emph{discriminate} between correct and incorrect AI answers, independent of their overall tendency to trust. We ask: when the AI is correct, does the user recognize it? When the AI is incorrect, does the user catch it? Following Schemmer et al.'s operationalization of appropriate reliance~\cite{schemmer2022should} and Buçinca et al.'s measurement of over-reliance~\cite{bucinca2021trust}, we define:

\begin{table}[h]
\centering
\small
\begin{tabular}{lcc}
\toprule
 & \textbf{User judged correct} & \textbf{User judged incorrect} \\
\midrule
\textbf{AI actually correct}   & $\text{correct-judgement}_{\text{correct}}$  & $\text{mis-judgement}_{\text{correct}}$ \\
\textbf{AI actually incorrect} & $\text{mis-judgement}_{\text{incorrect}}$ & $\text{correct-judgement}_{\text{incorrect}}$ \\
\bottomrule
\end{tabular}
\caption{Judgment outcomes. Each row conditions on AI correctness: the top row includes only items where the AI was correct; the bottom row includes only items where the AI was incorrect. }
\label{tab:judgment-matrix}
\end{table}

\begin{itemize}
    \item $\mathbf{correct-judgment_{\textbf{correct}}}$ $= \frac{|\{\text{AI actually correct} \cap \text{user judged as correct}\}|}{|\{\text{AI actually correct}\}|}$.
    Of all the items where the AI was actually correct, the fraction that the user correctly identified as correct. A high rate means the user is good at recognizing correct AI answers. This is equivalent to Schemmer et al.'s Relative AI Reliance (RAIR).

    \item $\mathbf{mis-judgement_{\textbf{correct}}}$ $= \frac{|\{\text{AI actually correct} \cap \text{user judged as incorrect}\}|}{|\{\text{AI actually correct}\}|}$.
    Of all the items where the AI was actually correct, the fraction that the user incorrectly rejected. A high rate means the user is failing to accept good AI answers---this captures under-reliance. $\text{correct-judgement}_{\text{correct}}$ and $\text{mis-judgement}_{\text{correct}}$ are complements and sum to one.

    \item $\mathbf{correct-judgment_{\textbf{incorrect}}}$ $= \frac{|\{\text{AI actually incorrect} \cap \text{user judged as incorrect}\}|}{|\{\text{AI actually incorrect}\}|}$.
    Of all the items where the AI was actually incorrect, the fraction that the user correctly identified as incorrect. A high rate means the user is good at catching AI errors. This is equivalent to Schemmer et al.'s Relative Self-Reliance (RSR).

    \item $\mathbf{mis-judgement_{\textbf{incorrect}}}$ $= \frac{|\{\text{AI actually incorrect} \cap \text{user judged as correct}\}|}{|\{\text{AI actually incorrect}\}|}$.
    Of all the items where the AI was actually incorrect, the fraction that the user incorrectly accepted as correct. A high rate means the user is being fooled by wrong AI answers---this is the over-reliance rate~\cite{bucinca2021trust}. $\text{correct-judgement}_{\text{incorrect}}$ and $\text{mis-judgement}_{\text{incorrect}}$ are complements and sum to one.
\end{itemize}

These metrics capture whether an explanation helps users distinguish correct from incorrect AI outputs, independent of the user's overall tendency to trust. An explanation that simply makes users trust more will increase both $\text{correct-judgement}_{\text{correct}}$ and $\text{mis-judgement}_{\text{incorrect}}$. An explanation that genuinely improves discrimination will increase $\text{correct-judgement}_{\text{correct}}$ while decreasing $\text{mis-judgement}_{\text{incorrect}}$.
\label{sec:eval-framework:judgement}

\subsubsection{Accuracy}
\begin{itemize}
    \item \textbf{Accuracy} $= \frac{|\{\text{user judged as correct} \cap \text{AI actually correct}\}| + |\{\text{user judged as incorrect} \cap \text{AI actually incorrect}\}|}{|\{\text{all judgments}\}|}$.
    The fraction of judgments where the user correctly identified whether the AI was right or wrong. This is the single measure of overall quality of the user's judgement of the AI's answers.
\end{itemize}

\subsection{Do variants of reasoning traces and post-hoc explanations engender false trust?}

Table~\ref{correct_and_false} reports, for each condition, the percentage of responses where the user judged the AI's answer to be correct, along with the true trust and false trust rates (as defined in Section~\ref{sec:eval-framework:trust}).

As shown by Table~\ref{correct_and_false}, users are being persuaded into believing a greater number of LLM generated answers as correct when exposed to reasoning traces and post-hoc LLM generated explanations. This would have been a positive result if the false trust rates associated with these conditions were low. However, we see that the \texttt{e\_plus} condition has a relatively high false trust rate across conditions.\footnote{The \texttt{solution\_only} condition has the highest false trust but we believe it is because the users have limited domain knowledge and thus are unable to distinguish between a correct and an incorrect answer when exposed only to the LLM generated answer.} The number of responses where the user was led into believing that an incorrect LLM generated response is correct is very high in the \texttt{e\_plus} condition. On the other hand, the \texttt{e\_dual} condition is more calibrated. Since the AI's accuracy in the task is 50\%, the rate of responses judged as correct is closest to the ground truth in the \texttt{e\_dual} condition. Among the responses judged as correct, the \texttt{e\_dual} condition has the lowest false trust rate (40.9\%), and thus, exposing the user to the merits and demerits of an answer helps in reducing the false trust engendered in the user.

\begin{table}[h]
\centering
\begin{tabular}{lcc}
\toprule
Condition & Responses judged as correct (True + False Trust) (\%) & False Trust (\%) \\
\midrule
\texttt{e\_dual}            & 57.3 & 40.9 \\
\texttt{e\_plus}            & 66.0 & 43.9 \\
\texttt{reasoning\_summary} & 58.5 & 43.6 \\
\texttt{reasoning\_trace}   & 64.5 & 41.9 \\
\texttt{solution\_only}     & 57.3 & 47.3 \\
\bottomrule
\end{tabular}
\caption{Percentage of responses judged as correct (the sum of true trust and false trust instances), and the false trust rate per explanation condition.}
\label{correct_and_false}
\end{table}
\subsection{Can users discriminate between correct and incorrect AI answers?}

In this section, we report how well users can discriminate between correct and incorrect AI answers across explanation conditions. We report $\text{correct-judgement}_{\text{correct}}$ (the rate at which users accept correct AI answers) and $\text{mis-judgement}_{\text{incorrect}}$(the rate at which users accept incorrect AI answers) in Table~\ref{tab:headline}).

The \texttt{e\_plus} and \texttt{reasoning\_trace} conditions achieve the highest $\text{correct-judgement}_{\text{correct}}$ rates (74.0\% and 75.0\% pooled, which implies that users in these conditions are good at recognizing correct AI answers. However, their $\text{mis-judgement}_{\text{incorrect}}$ rates are also high (58.0\% and 54.0\% pooled), meaning these explanations push users toward accepting AI answers indiscriminately, on both correct and incorrect items. This is the pattern described earlier in Section~\ref{sec:eval-framework:judgement}: an explanation that makes users trust more will increase both simultaneously.

\texttt{e\_dual} shows a different pattern. It achieves the lowest $\text{mis-judgement}_{\text{incorrect}}$ of any condition (46.9\% pooled) while maintaining a $\text{correct-judgement}_{\text{correct}}$ rate (67.7\%) that is above the \texttt{solution\_only} baseline (60.4\%). This is the only condition where users accept more correct answers \emph{and} reject more incorrect answers relative to \texttt{solution\_only}. \texttt{e\_dual} improves discrimination ability of the users than just shifting them towards trusting the AI answers.

\begin{table}[t]
\centering
\caption{$\text{correct-judgement}_{\text{correct}}$ (how often users accept correct AI answers) and $\text{mis-judgement}_{\text{incorrect}}$ (how often users accept incorrect AI answers) per explanation condition, split by item subset (fixed items shown to every participant; randomly sampled items drawn per participant; pooled = all 8 items). Cells are participant-mean rates in percent. \textbf{Bold} marks the best cell in each column (highest $\text{correct-judgement}_{\text{correct}}$, lowest $\text{mis-judgement}_{\text{incorrect}}$). $N_{\text{participants}}=24$--$25$ per condition.}
\label{tab:headline}
\small
\begin{tabular}{l rrr rrr}
\toprule
& \multicolumn{3}{c}{$\mathbf{correct-judgment_{\textbf{correct}}}$ ($\uparrow$)} & \multicolumn{3}{c}{$\mathbf{mis-judgement_{\textbf{incorrect}}}$ ($\downarrow$)} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
Condition & Fixed & Sampled & Pooled & Fixed & Sampled & Pooled \\
\midrule
\texttt{solution\_only}     & 56.2 & 64.6 & 60.4 & 60.4 & \textbf{47.9} & 54.2 \\
\texttt{e\_plus}            & 70.0 & \textbf{78.0} & 74.0 & 58.0 & 58.0 & 58.0 \\
\texttt{e\_dual}            & 66.7 & 68.8 & 67.7 & \textbf{45.8} & \textbf{47.9} & \textbf{46.9} \\
\texttt{reasoning\_summary} & 60.0 & 72.0 & 66.0 & 52.0 & 50.0 & 51.0 \\
\texttt{reasoning\_trace}   & \textbf{76.0} & 74.0 & \textbf{75.0} & 56.0 & 52.0 & 54.0 \\
\bottomrule
\end{tabular}
\end{table}

In the previous section, we noted that \texttt{solution\_only} has the highest false trust rate (47.3\%). Here we observe a similar pattern: without any explanation, users accept 60.4\% of correct answers but also accept 54.2\% of incorrect answers. This indicates that users with no explanation are not able to distinguish correct from incorrect AI outputs.

\begin{wraptable}{r}{0.35\textwidth}
\centering
\small
\begin{tabular}{l r}
\toprule
Condition & Acc. (\%) \\
\midrule
\texttt{solution\_only}     & 53.8 \\
\texttt{e\_plus}            & 58.3 \\
\texttt{e\_dual}            & \textbf{60.4} \\
\texttt{reasoning\_sum.}    & 56.2 \\
\texttt{reasoning\_trace}   & \textbf{60.4} \\
\bottomrule
\end{tabular}
\captionof{table}{Accuracy per condition (pooled).}
\label{tab:accuracy}
\end{wraptable}
 
(Table~\ref{tab:accuracy}) reports the accuracy across explanation conditions. \texttt{e\_dual} and \texttt{reasoning\_trace} tie for the highest accuracy (60.4\%), but they achieve this in fundamentally different ways. \texttt{reasoning\_trace} reaches 60.4\% through high $\text{correct-judgment}_{\text{correct}}$ (75.0\%) offset by high $\text{mis-judgment}_{\text{incorrect}}$ (54.0\%). Users accept most AI answers in this condition. \texttt{e\_dual} reaches the same accuracy through good $\text{correct-judgment}_{\text{correct}}$ (67.7\%) combined with the lowest $\text{mis-judgment}_{\text{incorrect}}$ of any condition (46.9\%).


\subsection{How does Trust and Judgement change across explanation conditions with different user knowledge?}

Before seeing the AI's answer, participants rated their familiarity with each problem (``I know the answer immediately,'' ``I might be able to solve it given more time,'' or ``I cannot solve this'').

Of the responses where users claimed to know the answer immediately, only 37\% were actually correct (33 of 90). We verified this by comparing users' own answers against the answer key (Table~\ref{tab:knowledge-verified}). Users who claimed knowledge and were actually correct achieved just 26.3\% $\text{mis-judgement}_{\text{incorrect}}$ and 84.8\% accuracy. Users who claimed knowledge but answered incorrectly showed 52.0\% $\text{mis-judgement}_{\text{incorrect}}$, no better than users who reported being unable to solve the problem at all (56.9\%). 

We now look at Table~\ref{tab:knowledge} which reports false trust rates, $\text{mis-judgement}_{\text{incorrect}}$, and accuracy for
different explanation conditions for users grouped by their knowledge of the problem.
\begin{table}[t]
\centering
\caption{Accuracy and $\text{mis-judgement}_{\text{incorrect}}$ by knowledge subgroup (pooled across conditions). ``Actually correct'' and ``actually wrong'' are subgroups of users who claimed to know the answer immediately, split by whether their own answer matched the answer key.}
\label{tab:knowledge-verified}
\small
\begin{tabular}{l r rr}
\toprule
Knowledge subgroup & $N$ & $\text{mis-judgement}_{\text{incorrect}}$ & Accuracy \\
\midrule
Claimed knowledge, actually correct & 33 & \textbf{26.3} & \textbf{84.8} \\
Claimed knowledge, actually wrong   & 57 & 52.0 & 66.7 \\
Might be able to solve it           & 449 & 51.9 & 57.2 \\
Cannot solve this                   & 413 & 56.9 & 55.2 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering
\caption{False trust, $\text{mis-judgement}_{\text{incorrect}}$, and accuracy for each condition compared by self-reported knowledge level. $N$ = item responses per subgroup. Before seeing the AI's answer, participants were asked: ``Do you know how to solve this question?'' (1 = ``I know the answer immediately,'' 2 = ``I might be able to solve it given more time,'' 3 = ``I cannot solve this'').}
\label{tab:knowledge}
\small
\begin{tabular}{l l r ccc}
\toprule
Knowledge Level & Condition & $N$ & False Trust (\%) & $\text{mis-judgement}_{\text{incorrect}}$ (\%) & Accuracy (\%) \\
\midrule
\multirow{5}{*}{I know it}
  & \texttt{e\_dual}            & 13 & 28.6 & 40.0 & 61.5 \\
  & \texttt{e\_plus}            & 13 & 33.3 & 42.9 & 76.9 \\
  & \texttt{reasoning\_summary} & 20 & 21.4 & 30.0 & 79.2 \\
  & \texttt{reasoning\_trace}   & 11 & 33.3 & 75.0 & 63.6 \\
  & \texttt{solution\_only}     & 33 & 29.2 & 38.9 & 80.0 \\
\midrule
\multirow{5}{*}{\shortstack[l]{I might solve it\\but need time}}
  & \texttt{e\_dual}            & 89 & 35.7 & \textbf{33.3} & \textbf{64.0} \\
  & \texttt{e\_plus}            & 99 & 37.3 & 54.5 & 61.0 \\
  & \texttt{reasoning\_summary} & 80 & 44.9 & 60.0 & 51.8 \\
  & \texttt{reasoning\_trace}   & 87 & 41.3 & 56.8 & 61.7 \\
  & \texttt{solution\_only}     & 94 & 51.0 & 56.5 & 47.4 \\
\midrule
\multirow{5}{*}{\shortstack[l]{I do not know\\how to solve}}
  & \texttt{e\_dual}            & 90 & 45.9 & 60.9 & 56.7 \\
  & \texttt{e\_plus}            & 80 & 53.6 & 64.4 & 51.2 \\
  & \texttt{reasoning\_summary} & 92 & 48.1 & 51.0 & 57.0 \\
  & \texttt{reasoning\_trace}   & 94 & 43.9 & 52.1 & 58.9 \\
  & \texttt{solution\_only}     & 57 & 54.3 & 57.1 & 46.7 \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{For users who know how to solve the problem : }When users know how to solve the problem and can confidently reach the solution, the need for explanation reduces~\citep{}. Knowledgeable users can confidently verify whether the given AI prediction is correct or not without requiring any assistance in the form of an explanation [CITE]. 
 This is reflected by the highest accuracy in the \texttt{solution\_only} condition (80.0\%). We also see that knowledgeable users, when displayed only the summary of the reasoning trace, can achieve very high accuracy (79.2\%) while minimizing $\text{mis-judgement}_{\text{incorrect}}$ (30.0\%).

However, \texttt{reasoning\_trace} is the only condition where higher knowledge does not help the user discriminate correct from incorrect AI answers. Among users who reported knowing the answer immediately, $\text{mis-judgement}_{\text{incorrect}}$ is 75.0\% which is higher than any other condition. We also note that \texttt{e\_plus} and \texttt{reasoning\_trace} shows 33.3\% false trust which is the highest among all conditions. More knowledgeable users appear to follow the reasoning traces more fluently, which makes it more convincing even when it leads to a wrong answer.

\paragraph{For users with partial knowledge : }
In cases where the users are not confident in their ability to solve the problem but have some domain knowledge, \texttt{e\_dual} achieves the lowest $\text{mis-judgement}_{\text{incorrect}}$ (33.3\%) and the highest accuracy (64.0\%), while also minimizing false trust as compared to other conditions.
This suggests that dual explanations are most effective when users have enough domain knowledge to evaluate the competing arguments. In contrast, the \texttt{reasoning\_summary} condition is the most detrimental for this group among the conditions where an explanation is provided. We observe that false trust rises to 44.9\%, $\text{mis-judgement}_{\text{incorrect}}$ rises to 60.0\% and accuracy drops to 51.8\%. Users with incomplete knowledge of the problem seem most susceptible to accepting an incorrect answer when a succint provenance explanation is provided along with it.

\paragraph{Users who cannot solve the problem.}
When users are completely unaware of how to solve the problem and are entirely reliant on the AI system, all explanation conditions improve accuracy over \texttt{solution\_only} (46.7\%). The \texttt{reasoning\_trace} and \texttt{reasoning\_summary} conditions perform well here (58.9\% and 57.0\% accuracy respectively). The \texttt{e\_dual} condition achieves similar accuracy to \texttt{reasoning\_summary} (56.7\%), but users are less likely to accept incorrect answers in the \texttt{e\_dual} condition as measured by false trust (45.9\% vs.\ 48.1\%). Thus, even for users with no domain knowledge, presenting the merits and demerits of an answer helps reduce the risk of the AI convincing users it is correct when it is actually wrong.

\subsection{Do users find all explanations equally helpful?}
\begin{table}[h]
\centering
\small
\begin{tabular}{llcccc}
\toprule
Helpfulness & Condition & $N$ (\%) & Perceived correct (\%) & Accuracy (\%) & False Trust (\%) \\
\midrule
\multirow{4}{*}{Helpful}
& \texttt{e\_dual}            & 72.4 & 59.7 & 64.0 & 36.1 \\
& \texttt{e\_plus}            & 83.0 & 69.3 & 59.6 & 42.6 \\
& \texttt{reasoning\_summary} & 64.0 & 77.3 & 57.0 & 44.4 \\
& \texttt{reasoning\_trace}   & 56.5 & 86.7 & 55.8 & 43.9 \\
\midrule
\multirow{4}{*}{Not Helpful}
& \texttt{e\_dual}            & 27.6 & 50.9 & 50.9 & 55.6 \\
& \texttt{e\_plus}            & 17.0 & 50.0 & 50.0 & 52.9 \\
& \texttt{reasoning\_summary} & 36.0 & 25.0 & 58.3 & 38.9 \\
& \texttt{reasoning\_trace}   & 43.5 & 35.6 & 66.7 & 35.5 \\
\bottomrule
\end{tabular}
\caption{Distribution of responses and behavioral metrics across conditions by perceived helpfulness. $N$ is the percentage of responses in each helpfulness group.}
\label{Tab:help}
\end{table}
After each question, across all conditions, participants rated whether the explanation helped them understand how the AI reached its answer. \texttt{solution\_only} provided no explanation and is omitted from this analysis.

Ironically, we find that the reasoning traces, supposedly the provenance explanations, were rated as least helpful with only 56.5\% of responses being rated as helpful, and the post-hoc \texttt{e\_plus} explanations, which were generated completely independently, were rated as most helpful for understanding how the AI reached its answer.

We further analyzed the users' responses based on whether they find an explanation to be helpful or not. When users find a reasoning trace or its summary to be helpful, they end up believing that the LLM reasoned correctly and thus its predicted answer must be correct. This is reflected in the high perceived correct rates. However, their accuracy does not reflect the same trend. The better the explanations become in convincing the user that the answer is correct, the worse the user becomes at detecting incorrect AI predictions, having higher false trust rates and lower accuracies. Ideally, we want explanations that are perceived as helpful by the users and help them distinguish between correct and incorrect LLM predictions. The \texttt{e\_dual} satisfies both requirements---it has a high helpful score (72.4\%) and among those responses, users have the highest accuracy (64.0\%) and lowest false trust (36.1\%).
%[CITE some work that points to user perceived helpfullness related to acceptance or trust]

\textcolor{red}{Reasoning traces and summaries generated on incorrect problems happen to mostly be perceived as not helpful by the users and thus, the users inherently begins to distrust the AI prediction [Maybe find a work to cite here]. This distrust works out in the users favour as the prediction happens to be wrong. Thus the higher prediction accuracy and the lower false trust rate cannot be used to say that explanation quality is good. But rather the explanation is so bad that the user begins to think that the answer must also be wrong. }

A significant number of questions (36\% and 43.6\%) have reasoning traces and their summaries that are perceived as not helpful by the users. We find that when users do not find these types of explanations to be helpful, their trust in the LLM generated predictions decreases, as indicated by the low perceived correct rates. This engendered distrust, due to the poor explanation quality, ends up being beneficial for the users as the majority of LLM predictions associated with these explanations are incorrect. Thus, the higher accuracy and lower false trust rates in the ``not helpful'' group should not be directly interpreted as evidence of higher explanation quality.

\subsection{Does self-reported trust predict accuracy of user judgment?}

After completing all items, participants rated their overall trust in the AI on a 7-point scale. We examine whether this self-reported trust measure predicts how well users actually judge the AI's answers.

Table~\ref{tab:trust-vs-calibration} splits participants by their self-reported trust level. Users who report higher trust show higher $\text{Correct Judgment}_{\text{correct}}$ (55.5\% to 89.6\%) and higher $\text{mis-judgement}_{\text{incorrect}}$ (39.0\% to 71.9\%). Self-reported trust predicts how often users say ``correct'' and not how often they are right. We find that self-reported trust has no correlation with accuracy (Pearson $r = 0.037$, $p = .686$) but is strongly correlated with $\text{mis-judgement}_{\text{incorrect}}$ ($r = 0.409$, $p < .001$). In other words, users who report trusting the AI more are not better at judging its answer. They simply accept more answers, correct and incorrect alike.

We find that \texttt{reasoning\_trace} elicits the highest self-reported trust (4.44/7) but has higher $\text{mis-judgement}_{\text{incorrect}}$ (54.0\%).
\texttt{e\_plus} follows the same pattern: second-highest self-reported trust (4.19/7) and the highest $\text{mis-judgement}_{\text{incorrect}}$ of any condition (58.0\%). Both formats provide one-sided reasoning and users respond by reporting high trust but accepting incorrect answers.
\texttt{e\_dual} elicits below-average self-reported trust (3.74/7) but achieves the lowest $\text{mis-judgement}_{\text{incorrect}}$ of any condition (46.9\%). If explanations were evaluated by user satisfaction alone, the format that produces the best user judgment would rank near the bottom. Self-reported trust measures how persuasive users found the explanation, not how well it actually helped them judge the AI's answers (Table~\ref{tab:trust-rankings}).

\begin{table}[t]
\centering
\caption{$\text{correct-judgment}_{\text{correct}}$, $\text{mis-judgment}_{\text{incorrect}}$, and accuracy split by self-reported trust level (post-study, 7-point scale, binned). $N$ = number of participants in that group.}
\label{tab:trust-vs-calibration}
\small
\begin{tabular}{l r rrr}
\toprule
Self-reported trust & $N$ & $\text{correct -judgment}_{\text{correct}}$ & $\text{mis-judgment}_{\text{incorrect}}$ & Accuracy \\
\midrule
Low (1--3)     & 43 & 55.5 & \textbf{39.0} & 58.2 \\
Medium (3.5--5) & 55 & 69.9 & 55.6 & 57.2 \\
High (5.5--7)  & 25 & \textbf{89.6} & 71.9 & \textbf{58.9} \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering
\caption{Conditions ranked by self-reported trust (post-study, 7-point scale) vs.\ actual $\text{mis-judgment}_{\text{incorrect}}$ and accuracy.}
\label{tab:trust-rankings}
\small
\begin{tabular}{l rrr}
\toprule
Condition & Self-reported trust & $\text{mis-judgment}_{\text{incorrect}}$ ($\downarrow$) & Accuracy ($\uparrow$) \\
\midrule
\texttt{reasoning\_trace}   & \textbf{4.44} & 54.0 & \textbf{60.5} \\
\texttt{e\_plus}            & 4.19 & 58.0 & 58.0 \\
\texttt{e\_dual}            & 3.74 & \textbf{46.9} & 60.4 \\
\texttt{reasoning\_summary} & 3.68 & 51.0 & 57.5 \\
\texttt{solution\_only}     & 3.67 & 54.2 & 53.1 \\
\bottomrule
\end{tabular}
\end{table}

